FedScalar: Federated Learning with Scalar Communication for Bandwidth-Constrained Networks

In bandwidth-constrained federated learning~(FL) settings, the repeated upload of high-dimensional model updates from agents to a central server constitutes the primary bottleneck, often rendering standard FL infeasible within practical communication budgets. We propose \emph{FedScalar}, a communication-efficient FL algorithm in which each agent uploads only two scalar values per round, regardless of the model dimension~$d$. Each agent encodes its local update difference as an inner product with a locally generated random vector and transmits the resulting scalar together with the generating seed, enabling the server to reconstruct an unbiased gradient estimate without any high-dimensional transmission. We prove that \emph{FedScalar} achieves a convergence rate of $O(d/\sqrt{K})$ to a stationary point for smooth non-convex loss functions, and show that adopting a Rademacher distribution for the random vector reduces the aggregation variance compared to the Gaussian case. Numerical simulations confirm that the dimension-free upload cost translates into significant improvements in wall-clock time and energy efficiency over \emph{FedAvg} and \emph{QSGD} in bandwidth-constrained settings.

==> intro1.tex <==
\section{Introduction}
In recent years, Federated Learning (FL)~\cite{HBM-EM-DR-SH-BAA:17} has emerged as a promising approach for distributed machine learning and optimal decision making for dynamical systems \cite{shiri2020communication, zeng2022federated}. FL has been successfully applied to a wide range of real-world applications \cite{hao2020apple, li2020webank}. In FL, collaborative learning is achieved without direct data sharing. Each agent receives the current model parameters from a central server and independently updates the model using its own dataset, as described in \cite{RX-SK-UAK:20}. The agents then send their locally updated model parameters back to the server, which typically combines them using a simple averaging method like the FedAvg algorithm \cite{HBM-EM-DR-SH-BAA:17}. The updated global model is redistributed to the agents, and this process is repeated iteratively until a satisfactory model is obtained. Figure~\ref{fig} illustrates a schematic representation of an FL architecture.



\begin{figure}[t]
\centering
    \includegraphics[scale=0.28]{Fig/schem.png}
    \caption{{\small Federated Learning structure where $\vect{x}$ represents the set of server's parameters}.}
    \label{fig}
\end{figure}
One of the main challenges in FL is the communication bottleneck between clients (agents) and the central server \cite{stoica2017berkeley, smith2017federated}. As illustrated in Fig.~\ref{fig}, training in FL is an iterative process involving two main phases in each iteration: downloading and uploading. During the downloading phase, the server sends the updated global model parameters to the clients. In the uploading phase, clients transmit their locally updated model parameters back to the server. Because clients must share high-dimensional model parameters and FL systems often involve millions of clients, the uploading process can cause significant transmission delays per training step, complicating model training. Additionally, in scenarios with limited communication resources, the time required to transmit FL parameters between clients and the server can exceed the time clients spend training their local models. Motivated by these challenges, designing communication-efficient FL algorithms is crucial. Such designs enable FL to scale to larger systems and generalize better while operating within the constraints of network communication resources.


Various methods have been proposed in the literature to address the communication challenges in FL. These solutions focus on optimizing agent scheduling, selection, and network resource management \cite{chen2018lag, yang2019scheduling, ren2020scheduling, rostami2023federated, li2020webank, mohri2019agnostic, chen2020convergence}. Other research efforts have reduced communication overhead by increasing local computation time \cite{jaggi2014communication, ma2017distributed, shamir2014communication, zhang2015disco}. A more recent study \cite{chen2021communication} proposed a method that jointly considers the impact of agent selection and network resource management.


In this paper, we propose a novel algorithm we term \texttt{FedScalar}, that significantly reduces communication between agents and the server when agents send back updated model parameters. Unlike existing communication-efficient algorithms that focus on device scheduling, selection, or network resource management, our approach requires agents to send only a single scalar value instead of a high-dimensional vector. 


To the best of our knowledge, this is the first work to systematically reduce communication costs by allowing agents to transmit only two scalar values to the server.  In the proposed algorithm, during the upload phase, each agent sends a single scalar computed as the inner product of its local update difference which represents the shift in the local model obtained after local stochastic gradient descent (SGD) steps together with a scalar seed value that allows the server to regenerate the same random vector used by the agent. The server then averages the received scalar values and decodes the information by projecting the scalar onto the regenerated random vector using the corresponding agent seed values.



Furthermore, we have rigorously shown that changing the underlying distribution of the random vector generated by the server can reduce the variance during the aggregation step of the proposed algorithm, specifically during the projection onto the random vector. We have demonstrated that the proposed algorithm achieves a convergence rate of $O(d/\sqrt{K})$ for smooth non-convex loss functions, significantly reducing communication overhead and making it well-suited for large-scale networks. Additionally, we validated the algorithm's performance across a range of datasets and machine learning~tasks.

\emph{Notations and terminologies}:  We let $\reals$, $\realpositive$, $\realnonnegative$, denote the set of real, positive real numbers. Consequently, when $x\in\real$, $|x|$ is its absolute value. For $\vect{x}\in\reals^d$,
$\|\vect{x}\|=\sqrt{\vect{x}^\top\vect{x}}$ denotes the standard Euclidean norm. We let $\langle.,.\rangle$ denotes an inner product between two vectors for two vectors $\vect{x}$ and $\vect{y}$ $\in \real^d$.
A differentiable function $f$: $\real^d \rightarrow \real$ is Lipschitz with constant $\mathsf{L}\in\real_{>0}$, or simply $\mathsf{L}$-Lipschitz, over a set $\mathcal{C} \subseteq \real^d$ if and only if $\|f(\vect{x})-f(\vect{y})\| \leq \mathsf{L} \|\vect{x}-\vect{y}\|$, for $\vect{x}, \vect{y} \in \mathcal{C}$. 
Lastly, we recall Jensen’s inequality, which states~\cite{DSB:09}:
\begin{align}
   \EX[\left \|\frac{1}{N}\sum\nolimits_{n=1}^{N}\!\vect{x}_n\right\|^2] &\leq \frac{1}{N}\sum\nolimits_{n=1}^{N} \EX[\|\vect{x}_n\|^2].%\\
  % \left \|\sum\nolimits_{n=1}^{N}x_n\right\|^2 &\leq N\sum\nolimits_{n=1}^{N}\|x_n\|^2.
\end{align}


\emph{Organization}: The remainder of this paper is organized as follows: %Section~\ref{sec::prelim} introduces our basic notation, and presents some of the properties of smooth functions. Section~\ref{se:problem-obj}presents the objective statement and the structure behind it.
Section \ref{se:problem-obj} presents the problem statement and formulation.
Section \ref{com-eff} includes the proposed algorithm and its steps and  contains our convergence analysis for the proposed algorithm and provides its convergence rate. This section presents also an in-depth analysis of the variance reduction in the proposed algorithm.
Section~\ref{sec::num} presents the effectiveness of our algorithm through simulation scenarios. Lastly, 
Section~\ref{sec::conclu} summarizes our conclusions and ideas for future
work. The proofs of the formal results are presented in the appendix. 



